Enhanced Online Test-time Adaptation with Feature-Weight Cosine Alignment

Online Test-Time Adaptation (OTTA) has emerged as an effective strategy to handle distributional shifts, allowing on-the-fly adaptation of pre-trained models to new target domains during inference, without the need for source data. We uncovered that the widely studied entropy minimization (EM) method for OTTA, suffers from noisy gradients due to ambiguity near decision boundaries and incorrect low-entropy predictions. To overcome these limitations, this paper introduces a novel cosine alignment optimization approach with a dual-objective loss function that refines the precision of class predictions and adaptability to novel domains. Specifically, our method optimizes the cosine similarity between feature vectors and class weight vectors, enhancing the precision of class predictions and the model's adaptability to novel domains. Our method outperforms state-of-the-art techniques and sets a new benchmark in multiple datasets, including CIFAR-10-C, CIFAR-100-C, ImageNet-C, Office-Home, and DomainNet datasets, demonstrating high accuracy and robustness against diverse corruptions and domain shifts.

==> figures/cifar_entropy_cos.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.98\linewidth]{figures/cifar10_entropy_cosine.pdf}
  \caption{Distribution comparisons of entropy and cosine similarity for CIFAR-10 against CIFAR-10-C under Gaussian noise corruption (severity level 5). Figures (A) and (B) illustrate the distribution of entropy and cosine similarity scores, respectively, across all samples, emphasizing the distributional shift induced by corruption. Figures (C) and (D) further dissect the entropy and cosine similarity within CIFAR-10-C, distinguishing between correctly and incorrectly classified samples, thus providing insight into the discriminative characteristics of the model's predictions in response to data corruption.}
  \label{fig:entropy_error}
\end{figure}

==> figures/comm_vs_em.tex <==
% \begin{figure}[t]
% \centering
% \begin{subfigure}[b]{0.9\textwidth}
%     \includegraphics[width=\textwidth]{figures/comm_vs_em/comm_vs_em_1.pdf}
%     \caption{A}
%     \label{fig:A}
% \end{subfigure}
% % \hfill % Adds horizontal space between figures
% % \begin{subfigure}[b]{0.49\textwidth}
% %     \includegraphics[width=\textwidth]{figures/comm_vs_em/comm_vs_em_2.pdf}
% %     \caption{B}
% %     \label{fig:B}
% % \end{subfigure}

% \caption{Three figures side by side.}
% \label{fig:three_figures}
% \end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.58\textwidth}
    \includegraphics[width=\textwidth]{figures/comm_vs_em/comm_vs_em_1.pdf}
    \caption{}
    \label{fig:comm_vs_em}
\end{subfigure}
    \hfill
\begin{subfigure}[t]{0.38\textwidth}
    \includegraphics[width=\textwidth]{figures/infograph/simplex_2d_all.pdf}
    \caption{}
    \label{fig:simplex_gradient}
\end{subfigure}
    \caption{(a) Comparison of the logit and softmax score adjustments pre-(blue) and post-(orange) optimization using entropy minimization (top) and CoMM (bottom) for `ship' class in CIFAR-10-C with brightness corruption level 5. (b) \hl{ADD CAPTION.}}
    % \vspace{-15pt}
    \label{fig:final}
\end{figure}

% Illustration of logits and softmax probabilities for a low-margin sample from the brightness corruption subset of CIFAR-10-C, class (8) ``ship''. The top row displays the changes induced by entropy minimization, while the bottom row showcases the impact of our proposed CoMM loss. Initially, high logits and softmax probabilities for classes 2 and 8 indicate a low-margin scenario (blue bars, labelled `Pre'). After optimization (orange bars, labelled `Post'), entropy minimization ambiguously increases the logits for multiple classes, whereas CoMM distinctly enhances the correct class, demonstrating a more targeted and effective adaptation.

==> inserts/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Ablation study comparing the performance of two cosine alignment criteria variants, namely $\mathcal{L}_\text{CoM}$ and $\mathcal{L}_\text{CoMM}$, against the entropy minimization method $\mathcal{L}_\text{EM}$ across three corruption benchmarks: CIFAR-10-C, CIFAR-100-C, and ImageNet-C. } %While CoM delivers performance on par with traditional entropy minimization approaches, CoMM further refines the adaptation process, leading to the lowest observed classification errors among the methods tested and showcasing its superior efficacy in handling corrupted data.}
\label{tab:ablation}
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{l|ccc}
\hline
\multirow{2}{*}{Methods} & \multicolumn{3}{c}{Classification Error (\%)} \\
                         & CIFAR-10-C    & CIFAR-100-C    & ImageNet-C   \\ \hline
$\mathcal{L}_\text{EM}$                   & 11.57         & 35.31          & 67.22        \\ 
$\mathcal{L}_\text{CoM}$                   & 11.10         & 35.28          & 67.77        \\
$\mathcal{L}_\text{CoMM}$                  & 10.14         & 32.75          & 62.33        \\ \hline
\end{tabular}%
}
\end{table}

==> inserts/batch_dependency.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{figures/batch_dependency.pdf}
    \caption{Performance comparison of TTA methods against varying batch sizes, showcasing our CoMM approach alongside entropy minimization techniques such as TENT and ETA. While TENT and ETA experience significant performance drops with batch sizes under 32, CoMM maintains a higher level of accuracy consistently across batch sizes, showing its resilience to batch size fluctuations.}
    \label{fig:batch_dependency}
\end{figure}

==> inserts/dual_plot.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/Entropies/entropies_pixelate.pdf} 
%         \caption{Impact of CoMM optimization on prediction entropy across training epochs on the ImageNet-C dataset with pixelate corruption.} %The graph demonstrates a clear downward trend in entropy, evidencing that the CoMM criterion not only aligns features with their respective class weight vectors but also concurrently minimizes prediction entropy, enhancing model certainty over time.}
%         \label{fig:cos_entropy_min}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.5\textwidth}
%         \centering
%     \includegraphics[width=\textwidth]{figures/batch_dependency.pdf}
%     \caption{Performance comparison of TTA methods against varying batch sizes, showcasing our CoMM approach alongside entropy minimization techniques such as TENT and ETA. While TENT and ETA experience significant performance drops with batch sizes under 32, CoMM maintains a higher level of accuracy consistently across batch sizes, showing its resilience to batch size fluctuations.}
%     \label{fig:batch_dependency}
%     \end{minipage}
% \end{figure}

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/Entropies/entropies_pixelate.pdf}
    \caption{} %The graph demonstrates a clear downward trend in entropy, evidencing that the CoMM criterion not only aligns features with their respective class weight vectors but also concurrently minimizes prediction entropy, enhancing model certainty over time.}
     \label{fig:cos_entropy_min}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.5\textwidth}
    \includegraphics[width=\textwidth]{figures/batch_dependency.pdf}
    \caption{}
    \label{fig:batch_dependency}
\end{subfigure}
\caption{(a) Impact of the proposed CoMM optimization on prediction entropy across training epochs on the ImageNet-C dataset with pixelate corruption. (b) Performance comparison of TTA methods against varying batch sizes, showcasing our CoMM approach alongside entropy minimization techniques such as TENT and ETA. While TENT and ETA experience significant performance drops with batch sizes under 32, CoMM maintains a higher level of accuracy consistently across batch sizes, showing its resilience to batch size fluctuations.}
\end{figure}


% \begin{minipage}{0.5\textwidth}
%         \centering
%         \caption{Ablation study comparing the performance of two cosine alignment criteria variants, namely $\mathcal{L}_\text{CoM}$ and $\mathcal{L}_\text{CoMM}$, against the entropy minimization method $\mathcal{L}_\text{EM}$ across three corruption benchmarks: CIFAR-10-C, CIFAR-100-C, and ImageNet-C. } 
%         \label{tab:ablation}
%         \resizebox{0.99\textwidth}{!}{%
%         \begin{tabular}{l|ccc}
%         \hline
%         \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Classification Error (\%)} \\
%                                  & CIFAR-10-C    & CIFAR-100-C    & ImageNet-C   \\ \hline
%         $\mathcal{L}_\text{EM}$                   & 11.57         & 35.31          & 67.22        \\ 
%         $\mathcal{L}_\text{CoM}$                   & 11.10         & 35.28          & 67.77        \\
%         $\mathcal{L}_\text{CoMM}$                  & 10.14         & 32.75          & 62.33        \\ \hline
%         \end{tabular}%
%         }        
%     \end{minipage}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \caption{Ablation study comparing the performance of two cosine alignment criteria variants, namely $\mathcal{L}_\text{CoM}$ and $\mathcal{L}_\text{CoMM}$, against the entropy minimization method $\mathcal{L}_\text{EM}$ across three corruption benchmarks: CIFAR-10-C, CIFAR-100-C, and ImageNet-C. } %While CoM delivers performance on par with traditional entropy minimization approaches, CoMM further refines the adaptation process, leading to the lowest observed classification errors among the methods tested and showcasing its superior efficacy in handling corrupted data.}
% \label{tab:ablation}
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l|ccc}
% \hline
% \multirow{2}{*}{Methods} & \multicolumn{3}{c}{Classification Error (\%)} \\
%                          & CIFAR-10-C    & CIFAR-100-C    & ImageNet-C   \\ \hline
% $\mathcal{L}_\text{EM}$                   & 11.57         & 35.31          & 67.22        \\ 
% $\mathcal{L}_\text{CoM}$                   & 11.10         & 35.28          & 67.77        \\
% $\mathcal{L}_\text{CoMM}$                  & 10.14         & 32.75          & 62.33        \\ \hline
% \end{tabular}%
% }
% \end{table}
